Validating IP Prefixes and AS-Paths with Blockchains

Networks (Autonomous Systems-AS) allocate or revoke IP prefixes with the intervention of official Internet resource number authorities, and select and advertise policy-compliant paths towards these prefixes using the inter-domain routing system and its primary enabler, the Border Gateway Protocol (BGP). Securing BGP has been a long-term objective of several research and industrial efforts during the last decades, that have culminated in the Resource Public Key Infrastructure (RPKI) for the cryptographic verification of prefix-to-AS assignments. However, there is still no widely adopted solution for securing IP prefixes and the (AS-)paths leading to them; approaches such as BGPsec have seen minuscule deployment. In this work, we design and implement a Blockchain-based system that (i) can be used to validate both of these resource types, (ii) can work passively and does not require any changes in the inter-domain routing system (BGP, RPKI), and (iii) can be combined with currently available systems for the detection and mitigation of routing attacks. We present early results and insights w.r.t. scalability.

==> tran_val.tex <==
Based on the \emph{IP Allocation} and \emph{BGP Path} transactions that are encoded --in sequence-- within the Blockchain (Sections~\ref{sec:tran-val:ip-allocation:types}, \ref{sec:tran-val:as-graph:types}) nodes/ASes recreate and update the corresponding states (Sections~\ref{sec:tran-val:ip-allocation:state}, \ref{sec:tran-val:as-graph:state}). Using these states, they validate transactions by comparing what they get with what they expect; if any transaction fails one of the checks, it is considered invalid, it is logged and is not accepted to be mined. Note that the creator of a transaction is always verified using cryptographic mechanisms, together with additional checks (\eg duplicate transactions are dropped for efficiency).

\myitemit{IP Allocation - Assign.} First, the node needs to check whether \texttt{as\_source} is able to assign this prefix to \texttt{as\_dest}; this is feasible only if (i) \texttt{as\_source} currently owns the prefix, (ii) it can provide the \texttt{txid} of the last valid assignment that transferred the prefix to it (\texttt{last\_assign}), (ii) its \texttt{source\_lease} is greater than (or equal to) the new\\\texttt{lease\_duration}, and (iii) it has the right to transfer the prefix to others (\texttt{transfer\_tag}). It also checks if the \texttt{as\_dest} are in the blockchain network; if not, they cannot be verified.

\myitemit{IP Allocation - Update.} The node first checks whether the lease of the current prefix owners has not already expired. It then checks if the AS that makes this transaction (\texttt{as\_source}) is the same as the one that made the original \emph{Assign} transaction (\texttt{assign\_tran}). Finally, it checks if the \texttt{as\_dest} in \texttt{assign\_tran}, currently own(s) the prefix. 

\myitemit{IP Allocation - Revoke.} The node needs to ensure that the lease has actually expired for revocation to be feasible. If it has expired, it also checks if the AS that makes this transaction (\texttt{as\_source}) is the same as the one that made the original \emph{Assign} transaction (\texttt{assign\_tran}). Finally, it checks if \texttt{as\_dest} in \texttt{assign\_tran}, currently own(s) the prefix.

\myitemit{BGP Path - Announce.} First, the node verifies the origin of this transaction (\texttt{as\_source}) based on the topology (AS-level graph) associated to this prefix; if \texttt{as\_source} does not have valid paths to the prefix via its \texttt{as\_source\_list} neighbors (from which it learned the prefix), the transaction is rejected. It then checks if all the ASes in \texttt{as\_source\_list} and \texttt{as\_dest\_list} are in the Blockchain network. Finally, it checks if this transaction introduces loops in the topology of this prefix; if it does, it is rejected.

\myitemit{BGP Path - Withdraw.}
Similarly to \emph{BGP Path - Announce} transaction checks, the node checks if there is at least one valid path from the withdrawing AS towards the prefix.

\myitem{Detecting Routing Attacks.}
Transactions that do not pass the aforementioned checks are considered invalid and are logged. These logs can be used to feed detection systems, either in real-time (\eg for automated countermeasures~\cite{sermpezis2018artemis}) or offline (\eg for forensic purposes). Depending on the type of invalid transaction, different alerts can be generated; \eg an invalid \emph{IP Allocation - Assign} transaction constitutes a ROA violation and potentially a fake origin hijack attempt. Invalid \emph{BGP Path - Announce} transactions may constitute path manipulation hijack attempts. Note that transactions in already mined blocks should also be checked for their validity. For example, assume that a node mines blocks with invalid transactions, either on purpose or due to a misconfiguration. Then, other nodes could potentially replace their chain with this one, if they validated only new broadcasted transactions without checking already mined ones. A solution to this problem is to mark all the invalid transactions as they happen. A new transaction must be broadcasted to all the nodes in the network so each one of them can verify whether it is valid or not. And thus, before replacing the chain, a node can look for all the invalid transactions it has marked in the incoming chain. If there is at least one invalid transaction in the new chain, the chain is rejected. Nodes that leave the network and come back or new nodes that join the network accept that the transactions in the current chain are all valid, deriving states accordingly.
